Exploratory Grasping: Asymptotically Optimal Algorithms for Grasping Challenging Polyhedral Objects

There has been significant recent work on data-driven algorithms for learning general-purpose grasping policies. However, these policies can consistently fail to grasp challenging objects which are significantly out of the distribution of objects in the training data or which have very few high quality grasps. Motivated by such objects, we propose a novel problem setting, Exploratory Grasping, for efficiently discovering reliable grasps on an unknown polyhedral object via sequential grasping, releasing, and toppling. We formalize Exploratory Grasping as a Markov Decision Process, study the theoretical complexity of Exploratory Grasping in the context of reinforcement learning and present an efficient bandit-style algorithm, Bandits for Online Rapid Grasp Exploration Strategy (BORGES), which leverages the structure of the problem to efficiently discover high performing grasps for each object stable pose. BORGES can be used to complement any general-purpose grasping algorithm with any grasp modality (parallel-jaw, suction, multi-fingered, etc) to learn policies for objects in which they exhibit persistent failures. Simulation experiments suggest that BORGES can significantly outperform both general-purpose grasping pipelines and two other online learning algorithms and achieves performance within 5% of the optimal policy within 1000 and 8000 timesteps on average across 46 challenging objects from the Dex-Net adversarial and EGAD! object datasets, respectively. Initial physical experiments suggest that BORGES can improve grasp success rate by 45% over a Dex-Net baseline with just 200 grasp attempts in the real world. See https://tinyurl.com/exp-grasping for supplementary material and videos.

==> 6-experiments.tex <==
\section{Experiments}
\label{sec:sim-exps}
In simulation experiments, we consider three questions: (1) Can \algabbr discover high quality grasps for which general-purpose grasping policies, such as Dex-Net 4.0~\cite{mahler2019learning} and GG-CNN~\citep{morrison2020learning}, perform poorly? (2) Does learning different policies for each stable pose accelerate grasp exploration? (3) Can \algabbr be applied in realistic settings in which objects may topple into new poses as a result of failed grasps? In Section~\ref{sec:phys-exps-supp} of the supplementary material we also present preliminary results indicating that in physical experiments on an ABB YuMi robot, \algabbr can significantly outperform a Dex-Net~\cite{mahler2019learning} baseline on two challenging 3D printed objects.
%Unfortunately due to the COVID-19 pandemic, we were unable to run physical experiments for the paper. However, since \algabbr samples grasps on image observations of the object and is evaluated in a similar simulation environment as used in~\citet{mahler2019learning}, which transferred learned grasping policies to physical bin picking environments, we expect that \algabbr can likely be extended to grasp exploration in the real world.

\subsection{Simulation Details}
\label{subsec:exp-setup}
To evaluate each policy, we choose 7 objects from the set of Dex-Net 2.0 adversarial objects~\cite{mahler2017dex} and 39 evaluation objects from the EGAD! dataset~\citep{morrison2020egad} for which general-purpose parallel-jaw grasping policies (Dex-Net 4.0~\cite{mahler2019learning} and GG-CNN~\cite{morrison2020learning}) perform poorly, despite there existing high-quality grasps in multiple stable poses. We sample a set of $K$ parallel-jaw grasps on the image observation of pose $s$ of each object as in~\cite{mahler2017dex}, and calculate the ground-truth quality of each grasp, $\phi_{s, a}$, using a wrench resistance metric that measures the ability of the grasp to resist gravity~\cite{mahler2018dex}. We randomize the initial pose of each object and execute \algabbr and baselines, sampling rewards from $\text{Ber}(\phi_{s, a})$. If the grasp succeeds, we randomize the pose, choosing a stable pose according to the stable pose distribution of the object. Otherwise, we assume that the object remains in the same stable pose. We execute each policy for 10 rollouts of 10 trials, where new grasps are sampled for each trial and each rollout evaluates the policy over 10,000 timesteps of grasp exploration. Since there is stochasticity in both the grasp sampling and the policies themselves, we average policy performance across the 10 rollouts and 10 trials. In addition, we smooth policy performance across a sliding window of 20 timesteps and report average reward for each timestep. 

To model object toppling when grasps are unsuccessful (Section~\ref{subsec:assumptions}), we use the toppling analysis from \citet{correa2019toppling} to determine the toppling transition matrix for a given object. Specifically, we generate the distribution of next states from a given state by sampling non-colliding pushes across vertices on the object, finding their distribution of next states given perturbations around the nominal push point, and average the distribution from all of the pushes. Then if a grasp fails, we choose the next state according to the corresponding topple transition probabilities. When evaluating policies, we remove poses that have no grasps with nonzero ground-truth quality and renormalize the stable pose distribution. We emphasize that we perform this step for all policies and do this only to ensure that no poses act as sink states from which the robot can never change the pose in the future (and thus ensure that Assumption~\ref{assum:ergodicity} is satisfied). For the 7 objects from the Dex-Net 2.0 adversarial object dataset, $11\%$ of poses (an average of 1.3 poses per object) were removed. We present additional experiments in the supplementary material where this pose removal step is not performed, and find that while all policies perform more poorly (Section~\ref{sec:additional-exps}), \algabbr still outperforms all baseline policies. We also include further details on the experimental setup in the supplementary material.

\subsection{Policies}
\label{subsec:policies}
We compare 3 variants of \algabbr against 3 baselines to evaluate whether \algabbr is able to (1) substantially outperform general-purpose grasping policies~\citep{mahler2019learning} on challenging objects and (2) learn more efficiently than other online learning algorithms which update a grasp quality convolutional network (GQCNN) online or explore grasps via reinforcement learning. We also instantiate \algabbr with different algorithms for $\mathcal{B}$ to study how this choice affects grasp exploration efficiency and implement an oracle baseline to study whether \algabbr is able to converge to the optimal policy. We compare the following baselines and Bandit Grasping variants: \textbf{Dex-Net}, which selects grasps greedily  with respect to the Grasp Quality Convolutional Network from Dex-Net 4.0~\cite{mahler2019learning} with probability $0.95$ and selects a grasp uniformly at random with probability $0.05$, \textbf{Dex-Net-FT}, which additionally fine tunes the GQCNN policy online from agent experience, an implementation of \textbf{UCRL2} from~\cite{UCRL_github}, a tabular RL algorithm discussed in Section~\ref{sec:rl}, and instantiations of \algabbr with the UCB-1 algorithm~\cite{auer2002finite} (\textbf{\algabbr-UCB}), Thompson sampling (\textbf{\algabbr-TS}) with a uniform Beta distribution prior, and Thompson sampling with a prior from the Dex-Net policy of strength 5 (\textbf{\algabbr-TS5}) as in~\cite{TSLP}. Finally, we implement an oracle baseline that chooses grasps with the best ground-truth metric at each timestep to establish an upper bound on performance.
% \begin{enumerate}
% [topsep=0pt,
% noitemsep,
% leftmargin=2pt,
% itemindent=12pt]
%     \item \textbf{GQCNN: }Selects grasps greedily with respect to the Grasp Quality Convolutional Network from Dex-Net 4.0~\cite{mahler2019learning} with probability $0.95$ and selects a grasp uniformly at random with probability $0.05$.
%     \item \textbf{GQCNNFT: }Same as GQCNN policy, but the GQCNN used for grasp quality evaluation is fine-tuned online based on grasp outcomes during policy execution.
%     \item \textbf{UCRL2: }The tabular reinforcement learning algorithm UCRL2~\cite{UCRL2}, implemented from~\cite{UCRL_github}.
%     \item \textbf{\algabbr (UCB): }We instantiate \algabbr with the no-regret online learning algorithm UCB-1~\cite{auer2002finite}.
%     \item \textbf{\algabbr (TS): }We instantiate \algabbr with the no-regret online learning algorithm Thompson Sampling~\cite{TS-regret}.
%     \item \textbf{\algabbr (TS-5): }We instantiate \algabbr with Thompson Sampling but use the GQCNN policy as a prior to accelerate exploration as in~\cite{TSLP}. 
%     \item \textbf{Optimal (Oracle): }We implement an oracle baseline which chooses grasps with the best ground-truth metric at each timestep.
% \end{enumerate}

% \subsection{Policy Learning without Toppling}
% \label{subsec:learning}
% We first evaluate the above baselines and \algabbr variants in a setting in which toppling is not possible ($\delta_{s, s'} = 0, \ \forall s \neq s$). This exacerbates the difficulty of grasp exploration since an object must be successfully grasped in a given pose for policies to be able to explore grasps in other poses. When evaluating policies without toppling, we remove poses that have no grasps with nonzero ground-truth quality and renormalize the stable pose distribution. We emphasize that we perform this step for all policies and do this only to ensure that no poses act as sink states from which the robot can never change the pose in the future (and thus ensure that Assumption~\ref{assum:ergodicity} is satisfied). For the 7 objects from the Dex-Net 2.0 adversarial object dataset, $11 \%$ of poses (an average of 1.3 poses per object) were removed. These poses made up an average of 2.8\% of the probability mass of the stable pose distribution.

% As shown in Figure~\ref{fig:policy_rewards}, the GQCNN policy typically performs very poorly, achieving an average reward of less than 0.1 per timestep. While the online learning policies also start poorly, they quickly improve, and \algabbr \textsc{(TS)} eventually converges to the optimal policy. We also find that \algabbr \textsc{(TS-5)}, which leverages GQCNN as a prior using the method presented in~\cite{TSLP}, further speeds convergence to the optimal policy. This result is promising, as it suggests that the exploration strategy in \algabbr can be flexibly combined with general-purpose grasping policies to significantly accelerate grasp exploration on unknown objects. We find that the GQCNNFT policy performs very poorly even though it continues to update the weights of the network online with the results of each grasp attempt and samples a random grasp with probability $0.05$, which aids exploration. We hypothesize that this is due to the initial poor performance of GQCNN---since the vast majority of fine-tuning grasps attain zero reward, the network is unable to explore enough high-quality grasps on the object. Overall, these results suggest that \algabbr can greatly increase grasp success rates on objects for which GQCNN performs poorly.
% \ashwin{@Mike, we should move no toppling row here to appendix}
% \begin{figure*}[htb!]
%     \centering
%     \includegraphics[width=\linewidth]{figures/rewards_v6.png}
%     \caption{\textbf{Simulation Experiments: }Performance of each policy across the vase, pawn and pipe objects from the Dex-Net 2.0 adversarial object set~\cite{mahler2017dex} (first three columns), as well as aggregated performance over the 7 Dex-Net objects (fourth column) and the 39 EGAD! objects (fifth column). We report the number of distinguishable stable poses ($S$) for each object, as well as its $\epsilon$ (ground truth value for the lowest quality best grasp across poses) and $\lambda_1$ (least likely stable pose probability) values, and show a top-down view of its three most likely stable poses. We report mean values of each metric for the datasets. The first row of plots shows reward over time for each policy in the original setting, where the object stays in the same pose until successfully grasped. The second row shows policy performance in the more realistic setting where the object may topple into an alternate pose when a grasp is unsuccessful. The value above each plot with toppling indicates the maximum difference in transitioning via toppling and transitioning via grasping to a new pose. In both cases, \algabbr quickly converges to optimal performance, while the other algorithms fail to reach optimal performance even after 10,000 grasp attempts. This result holds even when Assumption~\ref{assum:topple-bound} is violated.}
%     \label{fig:policy_rewards}
% \end{figure*}

% We also find that \algabbr policies greatly outperform the tabular RL policy UCRL2 by leveraging the structure of the grasp MDP. Both the UCB and Thompson sampling implementations maintain separate policies in each pose, thereby leveraging the fact that the optimal policy at each timestep is the greedy policy. This allows the \algabbr policies to not waste timesteps exploring the possible transitions to other states with low rewards. Thompson sampling additionally leverages the fact that the rewards are distributed as Bernoulli random variables, which may explain the significant performance gap between the Thompson sampling and UCB implementations. Thus, the \algabbr policies quickly learn to choose high-quality grasps in each pose and transition quickly to new, unexplored poses.

% We also perform sensitivity analysis of \algabbr to the grasp MDP parameters $\epsilon$ and $\lambda_1$ and find that \algabbr quickly converges to the optimal policy unless $\epsilon$ or $\lambda_1$ is low. In particular, we find that $\epsilon$ has an outsized effect on performance, which is intuitive given that $\epsilon$ affects the ability of \algabbr to both achieve immediate grasp successes \textit{and} explore new poses, while $\lambda_1$ only influences the latter. We additionally evaluate \algabbr for different numbers of sampled grasps ($K$) on each pose, and find that with decreasing values of $K$, all policies perform worse since the likelihood of sampling a high quality grasp decreases. However \algabbr policies continue to perform significantly better than prior methods and still achieve performance close to the optimal policies across a range of $K$s ($K = 10, 20, 50, 100, 200$). See Section~\ref{sec:sensitivity-exps} of the supplementary material for more details on sensitivity experiments.

% \subsection{Policy Learning with Toppling}
% We repeat the same experiments as in the previous section, with the additional condition that each object may now topple into another pose when a grasp is unsuccessful (Section~\ref{subsec:assumptions}). We use the toppling analysis from \citet{correa2019toppling} to determine the toppling transition matrix for a given object. Specifically, we generate the distribution of next states from a given state by sampling non-colliding pushes across vertices on the object, finding their distribution of next states given perturbations around the nominal push point, and average the distribution from all of the pushes. Then, during policy rollouts, if a grasp fails, we choose the next state according to the corresponding topple transition probabilities. See  the last row of Figure~\ref{fig:policy_rewards} for learning curves for \algabbr and baselines. Above the toppling experiment plots in the bottom row of Figure~\ref{fig:policy_rewards}, we report the maximum violation of Assumption~\ref{assum:topple-bound} across all object poses pairs for each object. Intuitively, this value captures how much more likely an object is to topple between poses $s$ and $s'$ than be successfully grasped $s$ and dropped into $s'$ for the pose pair $(s, s')$ which most violates Assumption~\ref{assum:topple-bound}. We find that \algabbr is robust even to large violations of Assumption~\ref{assum:topple-bound}, and substantially outperforms prior methods even when there exist pose pairs where it is $30\%$ more likely to topple between the poses than transition between them with a successful grasp.

\subsection{Experimental Results}
\label{subsec:exp-results}
Results for baselines and \algabbr variants are in Figure~\ref{fig:policy_rewards}. Above the learning curves in Figure~\ref{fig:policy_rewards}, we report the maximum violation of Assumption~\ref{assum:topple-bound} across all poses pairs for each object ($\max_{s,s'} \left[ \delta_{s,s'} - \epsilon\lambda_{s'}\right]$). This value captures how much more likely an object is to topple between poses $s$ and $s'$ than be successfully grasped in $s$ and released into $s'$ for pose pair $(s, s')$ which most violates Assumption~\ref{assum:topple-bound}. We find that \algabbr is robust to large violations of Assumption~\ref{assum:topple-bound}, and substantially outperforms prior methods even when there exist pose pairs where it is $30\%$ more likely to topple between the poses than transition between them with a successful grasp.

As shown in Figure~\ref{fig:policy_rewards}, the Dex-Net policy typically performs very poorly, achieving an average reward of less than 0.1 per timestep. While the online learning policies also start poorly, they quickly improve, and \algabbr-\textsc{TS} eventually converges to the optimal policy. We also find that \algabbr-\textsc{TS5}, which leverages Dex-Net as a prior using the method presented in~\cite{TSLP}, further speeds convergence to the optimal policy. This result is promising, as it suggests that the exploration strategy in \algabbr can be flexibly combined with general-purpose grasping policies to significantly accelerate grasp exploration on unknown objects. We find that the Dex-Net-FT policy performs very poorly even though it continues to update the weights of the network online with the results of each grasp attempt and samples a random grasp with probability $0.05$, which aids exploration. We hypothesize that this is due to the initial poor performance of Dex-Net---since the vast majority of fine-tuning grasps attain zero reward, the network is unable to explore enough high-quality grasps on the object. Overall, these results suggest that \algabbr can greatly increase grasp success rates on objects for which Dex-Net performs poorly. We also find that \algabbr policies greatly outperform tabular RL policy UCRL2 by leveraging the structure of the grasp MDP. Both the UCB and Thompson sampling implementations maintain separate policies in each pose, leveraging the fact that the optimal policy is the greedy policy. This allows the \algabbr policies to not waste timesteps exploring possible transitions to poses with low rewards. Thompson sampling additionally leverages the fact that the rewards are distributed as Bernoulli random variables, which may explain the significant performance gap between the Thompson sampling and UCB implementations. Thus, \algabbr policies quickly learn to choose high-quality grasps in each pose to transition quickly to new poses.

We perform sensitivity analysis of \algabbr to the grasp MDP parameters $\epsilon$ and $\lambda_1$ and find that \algabbr quickly converges to the optimal policy unless $\epsilon$ or $\lambda_1$ is low. In particular, we find that $\epsilon$ has an outsized effect on performance, which is intuitive given that $\epsilon$ affects the ability of \algabbr to both achieve immediate grasp successes \textit{and} explore new poses, while $\lambda_1$ only influences the latter. We additionally evaluate \algabbr for different numbers of sampled grasps ($K$) on each pose, and find that with decreasing values of $K$, all policies perform worse since the likelihood of sampling a high quality grasp decreases. However \algabbr policies continue to perform significantly better than prior methods and still achieve performance close to the optimal policies across a range of $K = \lbrace 10, 20, 50, 100, 200\rbrace$. See Section~\ref{sec:sensitivity-exps} of the supplementary material for more details.

% \section{Physical Experiments}
% \label{sec:phys-exps}
% We additionally evaluate \algabbr and the \textbf{GQCNN} baseline from Section~\ref{subsec:policies} in physical experiments on an ABB YuMi robot. (Figure \todo{insert}). We collect overhead depth images using a PhotoNeo PhoXi depth camera and sample a set of $K=$\ashwin{insert} parallel-jaw grasps on the image observation of pose $s$ of each object as in~\cite{mahler2017dex}. We find that \algabbr...  
% % Unfortunately due to the pandemic, we were unable to run physical experiments for the paper. However, since \algabbr samples grasps on image based observations of the object and is evaluated in a similar simulation environment as used in~\citet{mahler2018dex}, which transferred learned grasping policies to physical bin picking environments, we expect that \algabbr can likely be extended to grasp exploration in the real world.
% \ashwin{insert description and results}

==> 9-real-robot-discussion.tex <==
\clearpage
\setcounter{page}{1}
\resetlinenumber
\section*{COVID-19 and Physical Experiments}
\ashwin{update this if physical exps get done}
Due to the COVID-19 pandemic, the authors were unable to run physical experiments. However, \algabbr is developed in a similar simulation environment as Dex Net 4.0~\citecovid{mahler2019learning-covid}, which leveraged rendered simulated depth images to train a grasp quality CNN and was transferred to a physical setup. Thus, since like Dex Net 4.0, \algabbr also samples grasps on depth images rendered in a similar simulation environment, we expect that the grasp sampling procedure can easily be implement on a physical robotic system. 

Beyond grasp sampling, the key information that \algabbr assumes can be extracted from sensory input is (1) whether the object is in an unseen stable pose and (2) whether a grasp is successful. This is to ensure that (1) we can sample new grasps when a new stable pose is encountered and (2) supply \algabbr with an accurate reward signal. Determining grasp success from sensory information is a critical component of most prior work in robot grasping. In the bin picking setup, this can be done by using load cells to detect significant changes in weight as in~\citecovid{mahler2019learning-covid} while in other settings, standard object detection networks~\citecovid{zhao2019object-covid,tan2020efficientdet-covid,zhang2020resnest-covid} can be used to determine if the object is between the gripper jaws when they are lifted. To determine when a new object stable pose is encountered, the robot simply needs to be able to determine whether there exists a planar rotation/transition which explains the transformation between the current camera image and any prior captured image of the object. If such a transformation exists, then the object is not in a new stable pose and prior grasp samples can be rotated and translated onto the new image of the object. If not, then the object is in a new stable pose and new grasps must be sampled on the resulting image. We expect that a system can be implemented to recognize novel stable poses using prior work from point cloud registration~\citecovid{DGR-covid,wang2019deep-covid,zeng20173dmatch-covid}. We can use the resulting transformation to align the grasps sampled on the initial depth image to their respective poses in a later observation of the same stable pose. Finally, we realize that not all grasps that are sampled may be kinematically feasible for all translations and rotations of the object in the same stable pose. To avoid this issue, we can ensure that the object always lies within a region reachable by the robot arm using a shallow bin to constrain the object when it is dropped~\citecovid{mahler2019learning-covid}.

We are excited about applying \algabbr in physical experiments in future work, and will do so as soon as we are able to gain access to the robotics lab to conduct experiments. In physical experiments, we will implement a system that leverages prior work in point cloud registration to determine when a new stable pose is encountered and resample grasps on the depth image observation a new stable pose is detected using the same procedure as used for \algabbr in the main text. We will use load cells to determine whether grasp succeeds and otherwise implement the algorithms exactly as discussed in the main text. We will run the same experiments as in simulation, rolling out each policy for each test object in the Dex-Net 2.0 adversarial and EGAD datasets and capturing the average reward of the policy over time to directly compare policy performance.

\begin{small}
\bibliographystylecovid{corlabbrvnat}
\bibliographycovid{corl_covid}
\end{small}
